Evaluation Resolution Confounds Learning-Rule Comparisons in Model-Brain RSA of Early Visual Cortex

Revision note: see Comments. Studies of biologically plausible learning rules (feedback alignment, predictive coding, STDP) train small networks on $32\times32$ images and compare them with brain responses to naturalistic stimuli presented at much higher resolution. We find that a common result in this setting, that untrained or locally trained networks rival or beat backpropagation at early visual cortex, depends on the resolution at which networks are evaluated. In representational similarity analysis (RSA) against human V1, the gap between an untrained and a backprop-trained network grows monotonically from $-0.001$ (95% CI $[-0.011, 0.009]$) at the 32 px training resolution to $+0.030$ $[0.018, 0.042]$ at 224 px (six resolutions, 5 seeds; per-subject RSA on cross-run stimulus pairs). The growth reproduces for three further learning rules, directionally in single-seed macaque electrophysiology, along training, and for an ImageNet ResNet-50 and a Swin-Tiny transformer, which also align best at low resolution although trained at 224 px. Gabor and pixel structure, the normalization state of the untrained baseline, and a global brightness statistic do not account for it. Against a criterion fixed before the analysis, limiting image content to 32 px while the input still grows does not shrink the V1 gap ($+0.035$ $[0.023, 0.046]$ vs. $+0.030$ at 224 px; ratio 1.14 $[1.03, 1.34]$): it arises once the input exceeds the training resolution, through a decline of backprop. A single luminance value per image reaches rho= 0.054 against V1, matching the untrained network (0.053), which bounds what RSA on globally pooled features can resolve at V1 in this dataset. The one learning effect that holds across resolution is backprop above untrained at LOC. Comparisons of learning rules or architectures at early visual cortex need to control, and report, the evaluation resolution.

==> numbers_v3.tex <==
% generated by code/paper_v3/make_manifest.py -- do not edit
\makeatletter
\expandafter\def\csname nv@gap.V1.32\endcsname{-0.001}
\expandafter\def\csname nv@gap.V1.32.sem\endcsname{0.005}
\expandafter\def\csname nv@gap.V1.32.pos\endcsname{3}
\expandafter\def\csname nv@gap.V1.224\endcsname{+0.030}
\expandafter\def\csname nv@gap.V1.224.sem\endcsname{0.004}
\expandafter\def\csname nv@gap.V1.224.pos\endcsname{5}
\expandafter\def\csname nv@boot.V1.32.lo\endcsname{-0.011}
\expandafter\def\csname nv@boot.V1.32.hi\endcsname{0.009}
\expandafter\def\csname nv@boot.V1.224\endcsname{+0.030}
\expandafter\def\csname nv@boot.V1.224.lo\endcsname{0.018}
\expandafter\def\csname nv@boot.V1.224.hi\endcsname{0.042}
\expandafter\def\csname nv@gap.V1.64\endcsname{+0.010}
\expandafter\def\csname nv@gap.V1.64.pos\endcsname{3}
\expandafter\def\csname nv@gap.V1.96\endcsname{+0.018}
\expandafter\def\csname nv@gap.V1.96.pos\endcsname{5}
\expandafter\def\csname nv@gap.V1.128\endcsname{+0.023}
\expandafter\def\csname nv@gap.V1.128.pos\endcsname{5}
\expandafter\def\csname nv@gap.V1.160\endcsname{+0.026}
\expandafter\def\csname nv@gap.V1.160.pos\endcsname{5}
\expandafter\def\csname nv@mr.cr.V1.32\endcsname{-0.002}
\expandafter\def\csname nv@mr.cr.V1.224\endcsname{+0.042}
\expandafter\def\csname nv@mr.all.V1.224\endcsname{+0.043}
\expandafter\def\csname nv@mr.all.V1.32\endcsname{-0.001}
\expandafter\def\csname nv@rho.bp.V1.32\endcsname{0.046}
\expandafter\def\csname nv@rho.bp.V1.224\endcsname{0.023}
\expandafter\def\csname nv@rho.fa.V1.32\endcsname{0.015}
\expandafter\def\csname nv@rho.fa.V1.224\endcsname{0.009}
\expandafter\def\csname nv@rho.pc.V1.32\endcsname{0.019}
\expandafter\def\csname nv@rho.pc.V1.224\endcsname{0.012}
\expandafter\def\csname nv@rho.stdp.V1.32\endcsname{0.042}
\expandafter\def\csname nv@rho.stdp.V1.224\endcsname{0.027}
\expandafter\def\csname nv@rho.rnd.V1.32\endcsname{0.045}
\expandafter\def\csname nv@rho.rnd.V1.224\endcsname{0.053}
\expandafter\def\csname nv@bestgap.32\endcsname{+0.011}
\expandafter\def\csname nv@bestgap.32.sem\endcsname{0.004}
\expandafter\def\csname nv@bestgap.32.pos\endcsname{4}
\expandafter\def\csname nv@bestgap.96\endcsname{+0.030}
\expandafter\def\csname nv@bestgap.96.pos\endcsname{5}
\expandafter\def\csname nv@bestgap.224\endcsname{+0.042}
\expandafter\def\csname nv@bestgap.224.sem\endcsname{0.003}
\expandafter\def\csname nv@bestgap.224.pos\endcsname{5}
\expandafter\def\csname nv@gap.LOC.32\endcsname{+0.012}
\expandafter\def\csname nv@gap.LOC.32.sem\endcsname{0.001}
\expandafter\def\csname nv@gap.LOC.224\endcsname{+0.011}
\expandafter\def\csname nv@gap.LOC.224.sem\endcsname{0.001}
\expandafter\def\csname nv@gap.IT.32\endcsname{+0.012}
\expandafter\def\csname nv@gap.IT.32.sem\endcsname{0.001}
\expandafter\def\csname nv@gap.IT.224\endcsname{+0.006}
\expandafter\def\csname nv@gap.IT.224.sem\endcsname{0.001}
\expandafter\def\csname nv@rho.bp.LOC.32\endcsname{0.011}
\expandafter\def\csname nv@rho.bp.LOC.224\endcsname{0.008}
\expandafter\def\csname nv@rnd.LOC.max\endcsname{-0.001}
\expandafter\def\csname nv@rnd.LOC.min\endcsname{-0.003}
\expandafter\def\csname nv@cal.b-random.224\endcsname{-0.003}
\expandafter\def\csname nv@cal.b-random.224.sem\endcsname{0.006}
\expandafter\def\csname nv@cal.b-random.224.pos\endcsname{2}
\expandafter\def\csname nv@cal.d-random.224\endcsname{-0.009}
\expandafter\def\csname nv@cal.d-random.224.sem\endcsname{0.004}
\expandafter\def\csname nv@cal.d-random.224.pos\endcsname{2}
\expandafter\def\csname nv@cal.a-random.224\endcsname{-0.019}
\expandafter\def\csname nv@cal.a-random.224.sem\endcsname{0.004}
\expandafter\def\csname nv@cal.a-random.224.pos\endcsname{0}
\expandafter\def\csname nv@cal.c-random.224\endcsname{-0.014}
\expandafter\def\csname nv@cal.c-random.224.sem\endcsname{0.004}
\expandafter\def\csname nv@cal.c-random.224.pos\endcsname{0}
\expandafter\def\csname nv@cal.B-A.224\endcsname{+0.016}
\expandafter\def\csname nv@cal.B-A.224.sem\endcsname{0.004}
\expandafter\def\csname nv@cal.B-A.224.pos\endcsname{5}
\expandafter\def\csname nv@cal.D-C.224\endcsname{+0.006}
\expandafter\def\csname nv@cal.D-C.224.sem\endcsname{0.001}
\expandafter\def\csname nv@cal.D-C.224.pos\endcsname{5}
\expandafter\def\csname nv@cal.D-B.224\endcsname{-0.006}
\expandafter\def\csname nv@cal.D-B.224.sem\endcsname{0.004}
\expandafter\def\csname nv@cal.D-B.224.pos\endcsname{2}
\expandafter\def\csname nv@cal.b-bp.224\endcsname{+0.027}
\expandafter\def\csname nv@cal.b-bp.224.sem\endcsname{0.005}
\expandafter\def\csname nv@cal.b-bp.224.pos\endcsname{5}
\expandafter\def\csname nv@cal.d-bp.224\endcsname{+0.022}
\expandafter\def\csname nv@cal.d-bp.224.sem\endcsname{0.001}
\expandafter\def\csname nv@cal.d-bp.224.pos\endcsname{5}
\expandafter\def\csname nv@cal.sem.min\endcsname{0.001}
\expandafter\def\csname nv@cal.sem.max\endcsname{0.005}
\expandafter\def\csname nv@arch.resnet50.32\endcsname{0.031}
\expandafter\def\csname nv@arch.resnet50.224\endcsname{0.023}
\expandafter\def\csname nv@arch.swin_t.32\endcsname{0.056}
\expandafter\def\csname nv@arch.swin_t.224\endcsname{0.037}
\expandafter\def\csname nv@ref.lum.V1\endcsname{0.054}
\expandafter\def\csname nv@ref.hist.V1\endcsname{0.031}
\expandafter\def\csname nv@ref.rgb.V1\endcsname{0.020}
\expandafter\def\csname nv@ref.pixel.V1\endcsname{0.020}
\expandafter\def\csname nv@gabor.V1.min\endcsname{0.012}
\expandafter\def\csname nv@gabor.V1.max\endcsname{0.027}
\expandafter\def\csname nv@unt.partial_lum\endcsname{0.026}
\expandafter\def\csname nv@unt.pixel_decrease\endcsname{0.002}
\expandafter\def\csname nv@gap.joint4.32\endcsname{-0.013}
\expandafter\def\csname nv@gap.joint4.224\endcsname{+0.024}
\expandafter\def\csname nv@gap.lum.224\endcsname{+0.017}
\expandafter\def\csname nv@six.order\endcsname{0.94}
\expandafter\def\csname nv@within.rho25\endcsname{0.87}
\expandafter\def\csname nv@within.B.dV1\endcsname{+0.008}
\expandafter\def\csname nv@within.B.dV1.pos\endcsname{4}
\expandafter\def\csname nv@ups.step.bp\endcsname{-0.023}
\expandafter\def\csname nv@ups.step.rnd\endcsname{-0.000}
\expandafter\def\csname nv@ups.gapopen.NATIVE\endcsname{+0.021}
\expandafter\def\csname nv@ups.gapopen.NATIVE.sem\endcsname{0.001}
\expandafter\def\csname nv@ups.gapopen.NATIVE.pos\endcsname{5}
\expandafter\def\csname nv@ups.gapopen.UPSAMPLED\endcsname{+0.002}
\expandafter\def\csname nv@ups.gapopen.UPSAMPLED.sem\endcsname{0.001}
\expandafter\def\csname nv@ups.gapopen.UPSAMPLED.pos\endcsname{4}
\expandafter\def\csname nv@ups.bp.NATIVE\endcsname{-0.016}
\expandafter\def\csname nv@ups.bp.NATIVE.sem\endcsname{0.001}
\expandafter\def\csname nv@ups.bp.UPSAMPLED\endcsname{-0.000}
\expandafter\def\csname nv@ups.bp.UPSAMPLED.sem\endcsname{0.001}
\expandafter\def\csname nv@ups.bp.UPSAMPLED.pos\endcsname{2}
\expandafter\def\csname nv@ups.fa.NATIVE\endcsname{-0.003}
\expandafter\def\csname nv@ups.fa.UPSAMPLED\endcsname{+0.002}
\expandafter\def\csname nv@ups.pc.NATIVE\endcsname{-0.003}
\expandafter\def\csname nv@ups.pc.UPSAMPLED\endcsname{+0.003}
\expandafter\def\csname nv@ups.rnd.UPSAMPLED\endcsname{+0.0021}
\expandafter\def\csname nv@ups.rnd.UPSAMPLED.sem\endcsname{0.0002}
\expandafter\def\csname nv@ups.rnd.frac\endcsname{44}
\expandafter\def\csname nv@ups.removed\endcsname{89}
\expandafter\def\csname nv@td.bp.224\endcsname{-0.030}
\expandafter\def\csname nv@td.bp.224.sem\endcsname{0.005}
\expandafter\def\csname nv@td.bp.224.neg\endcsname{5}
\expandafter\def\csname nv@td.bp.32\endcsname{+0.001}
\expandafter\def\csname nv@td.bp.32.sem\endcsname{0.005}
\expandafter\def\csname nv@td.bp.32.neg\endcsname{3}
\expandafter\def\csname nv@td.pc.32\endcsname{-0.025}
\expandafter\def\csname nv@td.pc.32.sem\endcsname{0.004}
\expandafter\def\csname nv@td.fa.32\endcsname{-0.021}
\expandafter\def\csname nv@td.fa.32.sem\endcsname{0.007}
\expandafter\def\csname nv@p1.rnd\endcsname{0.053}
\expandafter\def\csname nv@p1.bp\endcsname{0.022}
\expandafter\def\csname nv@p1.gap\endcsname{+0.031}
\expandafter\def\csname nv@p1.gap.lo\endcsname{0.019}
\expandafter\def\csname nv@p1.gap.hi\endcsname{0.043}
\expandafter\def\csname nv@p1.pr.min\endcsname{0.002}
\expandafter\def\csname nv@p1.pr.max\endcsname{0.005}
\expandafter\def\csname nv@lb.V1\endcsname{0.051}
\expandafter\def\csname nv@lb.V2\endcsname{0.024}
\expandafter\def\csname nv@lb.LOC\endcsname{0.018}
\expandafter\def\csname nv@lb.IT\endcsname{0.021}
\expandafter\def\csname nv@lb.V1.lo\endcsname{0.039}
\expandafter\def\csname nv@lb.V1.hi\endcsname{0.064}
\expandafter\def\csname nv@s4.V1.up224\endcsname{+0.035}
\expandafter\def\csname nv@s4.V1.up224.lo\endcsname{0.023}
\expandafter\def\csname nv@s4.V1.up224.hi\endcsname{0.046}
\expandafter\def\csname nv@s4.V1.R\endcsname{1.14}
\expandafter\def\csname nv@s4.V1.R.lo\endcsname{1.03}
\expandafter\def\csname nv@s4.V1.R.hi\endcsname{1.34}
\expandafter\def\csname nv@s4.V1.diff\endcsname{+0.004}
\expandafter\def\csname nv@s4.V1.diff.lo\endcsname{0.001}
\expandafter\def\csname nv@s4.V1.diff.hi\endcsname{0.008}
\expandafter\def\csname nv@s4.LOC.up224\endcsname{+0.003}
\expandafter\def\csname nv@s4.LOC.up224.lo\endcsname{-0.004}
\expandafter\def\csname nv@s4.LOC.up224.hi\endcsname{0.009}
\expandafter\def\csname nv@s4.LOC.R\endcsname{0.23}
\expandafter\def\csname nv@s4.LOC.R.lo\endcsname{-0.58}
\expandafter\def\csname nv@s4.LOC.R.hi\endcsname{0.83}
\expandafter\def\csname nv@s4.LOC.diff\endcsname{-0.009}
\expandafter\def\csname nv@s4.LOC.diff.lo\endcsname{-0.017}
\expandafter\def\csname nv@s4.LOC.diff.hi\endcsname{-0.001}
\expandafter\def\csname nv@s4.V1.up64\endcsname{+0.032}
\expandafter\def\csname nv@s4.bp.up.min\endcsname{0.014}
\expandafter\def\csname nv@s4.bp.up.max\endcsname{0.016}
\expandafter\def\csname nv@s4.bp.up.64\endcsname{0.016}
\expandafter\def\csname nv@td.bp224.e0\endcsname{0.053}
\expandafter\def\csname nv@td.bp224.e1\endcsname{0.012}
\expandafter\def\csname nv@td.bp224.e40\endcsname{0.023}
\makeatother
\newcommand{\NV}[1]{\ifcsname nv@#1\endcsname\csname nv@#1\endcsname\else\errmessage{Undefined number: #1}\fi}

